Synergistic Offline-Online Control Synthesis via Local Gaussian Process Regression

Autonomous systems often have complex and possibly unknown dynamics due to, e.g., black-box components. This leads to unpredictable behaviors and makes control design with performance guarantees a major challenge. This paper presents a data-driven control synthesis framework for such systems subject to linear temporal logic on finite traces (LTLf) specifications. The framework combines a baseline (offline) controller with a novel online controller and refinement procedure that improves the baseline guarantees as new data is collected. The baseline controller is computed offline on an uncertain abstraction constructed using Gaussian process (GP) regression on a given dataset. The offline controller provides a lower bound on the probability of satisfying the LTLf specification, which may be far from optimal due to both discretization and regression errors. The synergy arises from the online controller using the offline abstraction along with the current state and new data to choose the next best action. The online controller may improve the baseline guarantees since it avoids the discretization error and reduces regression error as new data is collected. The new data are also used to refine the abstraction and offline controller using local GP regression, which significantly reduces the computation overhead. Evaluations show the efficacy of the proposed offline-online framework, especially when compared against the offline controller.

==> results/benchmark-global-static.tex <==
\begin{tabular}{ccccccccccc}
\hline
Exp. &  $x_0$ Index & Sec. & Success \% & Indet. \% & Avg. Steps & Avg. Comp. Time\\
\hline
online & $1.00$ & Sink+Prog & $1.00$ & $0.00$ & $39.20$  & $0.0002$\\
online & $1.00$ & Sink & $0.06$ & $0.46$ & $75.82$  & $0.0002$\\
% online & $1.00$ & none & $0.00$ & $0.00$ & $9.06$ & $0.00$\\
offline & $1.00$ & $-$ & $0.00$ & $0.00$ & $3.00$ & $0.00$\\
\hline
online & $2.00$ & Sink & $0.84$ & $0.16$ & $51.30$ & $0.0002$\\
online & $2.00$ & Sink+Prog & $0.78$ & $0.22$ & $28.52$ & $0.00$\\
% online & $2.00$ & none & $0.24$ & $0.00$ & $12.06$ & $0.00$\\
offline & $2.00$ & $-$ & $0.00$ & $0.00$ & $10.58$  & $0.00$\\
\hline
offline & $3.00$ & $-$ & $0.72$ & $0.00$ & $13.76$ & $0.00$\\
online & $3.00$ & Sink & $0.18$ & $0.82$ & $93.32$ & $0.0001$\\
% online & $3.00$ & none & $0.00$ & $0.00$ & $6.02$ & $0.00$\\
online & $3.00$ & Sink+Prog & $0.00$ & $1.00$ & $100.00$ & $0.0001$\
% online & $3.00$ & $dfa$ & $0.04$ & $51.84$ & $-$ & $0.00$ & $0.0008$ & $\infty$ & $0.0002$\\
% online & $3.00$ & none & $0.00$ & $5.56$ & $-$ & $0.00$ & $0.00$ & $\infty$ & $0.0001$\\
% online & $3.00$ & $dfa+pimdp$ & $0.00$ & $40.36$ & $-$ & $0.00$ & $0.00$ & $\infty$ & $0.0002$\\
% offline & $-$ & $3.00$ & $-$ & $0.00$ & $20.60$ &  - &  - & $\infty$ & $\infty$ & $0.00$\\
\end{tabular}


==> results/benchmark-global-update.tex <==
\begin{tabular}{ccccccccccc}
\hline
Exp. &  $x_0$ Index & Sec. & Prob. & Avg. Steps & Avg. $\policyoff$ Improv. & Avg. Trans. Improv. & Mean Prim & Mean Sec & Avg. Comp. Time\\
\hline

\end{tabular}

==> results/benchmark-local-static.tex <==
\begin{tabular}{ccccccccccc}
\hline
Exp. &  $x_0$ Index & Sec. & Success \% & Indet. \% & Avg. Steps & Avg. Comp. Time\\
\hline
online & $1.00$ & Sink+Prog & $1.00$ & $0.00$ & $39.66$ & $0.0003$\\
online & $1.00$ & Sink & $0.08$ & $0.52$ & $77.84$ & $0.0004$\\
% online & $1.00$ & none & $0.00$ & $0.00$ & $10.12$ & $0.0002$\\
\hline
offline & $1.00$ & $-$ & $0.00$ & $0.00$ & $3.00$ & $0.00$\\
online & $2.00$ & Sink & $0.88$ & $0.12$ & $48.28$ & $0.0002$\\
online & $2.00$ & Sink+Prog & $0.84$ & $0.16$ & $23.18$ & $0.0001$\\
% online & $2.00$ & none & $0.16$ & $0.00$ & $13.56$ & $0.0005$\\
offline & $2.00$ & $-$ & $0.00$ & $0.00$ & $10.98$ & $0.00$\\
\hline
offline & $3.00$ & $-$ & $0.70$ & $0.00$ & $13.84$ & $0.00$\\
online & $3.00$ & Sink & $0.08$ & $0.92$ & $96.96$ &  $0.0004$\\
% online & $3.00$ & none & $0.00$ & $0.00$ & $6.24$ &  $0.0001$\\
online & $3.00$ & Sink+Prog & $0.00$ & $0.98$ & $98.68$ & $0.0004$\\



% online & $1.00$ & $dfa+pimdp$ & $1.00$ & $10.32$ & $-$ & $0.00$ & $0.1090$ & $-2.1939$ & $0.0002$\\
% online & $1.00$ & $dfa$ & $0.84$ & $39.92$ & $-$ & $0.00$ & $0.0474$ & $-1.3472$ & $0.0002$\\
% online & $1.00$ & none & $0.16$ & $17.48$ & $-$ & $0.00$ & $0.0080$ & $\infty$ & $0.0006$\\
% offline& $1.00$ & $-$ & $0.00$ & $2.00$ & $-$ & $-$ & $\infty$ & $\infty$ & $0.00$\\
% \hline
% online & $2.00$ & $dfa$ & $0.80$ & $52.12$ & $-$ & $0.00$ & $0.0097$ & $-1.0831$ & $0.0004$\\
% online & $2.00$ & $dfa+pimdp$ & $0.72$ & $34.00$ & $-$ & $0.00$ & $0.10$ & $-1.7735$ & $0.0003$\\
% online & $2.00$ & none & $0.24$ & $17.52$ & $-$ & $0.00$ & $0.0093$ & $\infty$ & $0.0003$\\
% offline& $2.00$ & $-$ & $0.00$ & $10.52$ & $-$ & $-$ & $\infty$ & $\infty$ & $0.00$\\
% online & $3.00$ & $dfa$ & $0.04$ & $37.68$ & $-$ & $0.00$ & $0.00$ & $\infty$ & $0.0003$\\
% online & $3.00$ & none & $0.00$ & $4.16$ & $-$ & $0.00$ & $0.00$ & $\infty$ & $0.0002$\\
% online & $3.00$ & $dfa+pimdp$ & $0.00$ & $47.32$ & $-$ & $0.00$ & $0.00$ & $\infty$ & $0.0003$\\
% offline & $-$ & $3.00$ & $-$ & $0.00$ & $20.56$ & $-$ & $-$ & $\infty$ & $\infty$ & $0.00$\\
\end{tabular}


==> results/benchmark-local-update.tex <==
\begin{tabular}{ccccccccccc}
\hline
Exp. &  $x_0$ Index & Sec. & Success \% & Indet \% & Avg. Steps & Avg. \# Improv. & Avg. Trans. Change & Avg. Comp. Time\\
\hline
online & $1.00$ & Sink+Prog & $1.00$ & $0.00$ & $31.58$  & $640.50$ & $1.00$ & $0.0135$\\
online & $1.00$ & Sink & $0.10$ & $0.70$ & $82.92$ & $3362.40$ & $0.9996$ & $0.0323$\\
% online & $1.00$ & none& $0.00$ & $0.00$ & $10.38$ & $268.68$ & $-$ & $0.0175$\\
offline & $1.00$ & $-$ & $0.00$ & $0.00$ & $3.00$ & $-$ & $-$ & $0.00$\\
\hline
online & $2.00$ & Sink+Prog & $0.96$ & $0.04$ & $18.90$ & $118.44$ & $-$ & $0.0256$\\
online & $2.00$ & Sink & $0.86$ & $0.14$ & $56.40$ & $604.56$ & $-$ & $0.0151$\\
% online & $2.00$ & none& $0.28$ & $0.00$ & $13.62$ & $54.66$ & $-$ & $0.0243$\\
offline & $2.00$ & $-$ & $0.00$ & $0.00$ & $10.82$ &  $-$ & $-$ & $0.00$\\
\hline
offline & $3.00$ & $-$ & $0.68$ & $0.00$ & $13.96$ &  $-$ & $-$ & $0.00$\\
online & $3.00$ & Sink+Prog & $0.24$ & $0.70$ & $88.00$ & $1734.96$ & $0.9935$ & $0.0130$\\
online & $3.00$ & Sink & $0.06$ & $0.90$ & $96.24$ & $4192.92$ & $0.9960$ & $0.0120$\\
% online & $3.00$ & none& $0.00$ & $0.00$ & $6.74$ & $181.38$ & $-$ & $0.0123$\\
% \hline
% online & $1.00$ & $dfa+pimdp$ & $1.00$ & $10.84$ & $0.00$ & $0.48$ & $0.1071$ & $-2.2250$ & $0.0037$\\
% online & $1.00$ & $dfa$ & $0.88$ & $34.96$ & $0.00$ & $28.92$ & $0.0487$ & $\infty$ & $0.0028$\\
% online & $1.00$ & none& $0.12$ & $16.52$ & $0.00$ & $13.68$ & $0.0075$ & $\infty$ & $0.0030$\\
% offline & $1.00$ & $-$ & $0.00$ & $2.00$ & - & - & $\infty$ & $\infty$ & $0.00$\\
% \hline
% online & $2.00$ & $dfa$ & $0.92$ & $45.96$ & $0.00$ & $11.64$ & $0.0206$ & $-1.1090$ & $0.0023$\\
% online & $2.00$ & $dfa+pimdp$ & $0.92$ & $21.28$ & $0.00$ & $8.64$ & $0.1026$ & $-1.7625$ & $0.0034$\\
% online & $2.00$ & none& $0.24$ & $18.44$ & $0.00$ & $0.48$ & $0.0026$ & $\infty$ & $0.0026$\\
% offline& $2.00$ & $-$ & $0.00$ & $10.32$ & - & - & $\infty$ & $\infty$ & $0.00$\\
% online & $3.00$ & none& $0.00$ & $4.36$ & $0.00$ & $13.92$ & $0.00$ & $\infty$ & $0.0018$\\
% online & $3.00$ & $dfa$ & $0.00$ & $42.16$ & $0.0001$ & $466.44$ & $0.00$ & $\infty$ & $0.0012$\\
% online & $3.00$ & $dfa+pimdp$ & $0.00$ & $61.48$ & $0.00$ & $153.36$ & $0.00$ & $\infty$ & $0.0026$\\
% offline & $-$ & $3.00$ & $-$ & $0.00$ & $20.36$ & - & - & $\infty$ & $\infty$ & $0.00$\\
\end{tabular}


==> results/benchmark-megatable-old.tex <==
\begin{tabular}{cc|ccc|ccccc|ccc}
\multicolumn{2}{c}{}& \multicolumn{3}{c}{Global GP (static)} & \multicolumn{5}{c}{Local GP (updates with $K=75$ neighbors)} & \multicolumn{3}{c}{Local GP (static)}\\
\hline
$x_0$ & Tertiary & $P_\text{Violate}$ & $P_\text{Satisfy}$  & Time & $P_\text{Violate}$ & $P_\text{Satisfy}$  & Time & \# $\PIMDP$-updates & Val. $\PIMDP$-updates & $P_\text{Violate}$ & $P_\text{Satisfy}$  & Time \\
\hline
$1$ & Offline & $1.0$ & $0.0$ & $-$ & $1.0$ & $0.0$ & $-$ & $-$ & $-$ & $1.0$ & $0.0$ & $-$\\
$1$ & Sink+Prog & $0.0$ & $\mathbf{1.0}$ & $0.0002$ & $0.0$ & $\mathbf{1.0}$ & $0.0135$ & 640.5 & 1.0 & $0.0$ & $\mathbf{1.0}$ & $0.0003$\\
$1$ & Sink & $0.48$ & $\mathbf{0.46}$ & $0.0002$& $\mathbf{0.2}$ & $0.1$ & $0.0323$ &3362.4 & 0.9996 & $0.4$ & $0.08$ & $0.0004$ \\
\hline
$2$ & Offline & $1.00$ & $0.00$ & $-$ & $1.00$ & $0.00$ & $-$ & $-$ & $-$ & $1.00$ & $0.00$ & $-$ \\
$2$ & Sink+Prog & $0.0$ & $0.78$ & ($0.0001$)  & $0.0$ & $\mathbf{0.98}$ & $0.0222$ &160.86 & 1.0 & $0.0$ & $0.84$ & $0.0001$\\
$2$ & Sink & $0.0$ & $0.84$ & $0.0002$ & $0.0$ & $\mathbf{0.94}$ & $0.0115$ &334.02 & 0.9998 & $0.0$ & $0.88$ & $0.0002$\\
\hline
$3$ & Offline & $0.28$ & $\mathbf{0.72}$ & $-$ & $0.28$ & $\mathbf{0.72}$ & $-$ & $-$ & $-$ & $0.28$ & $\mathbf{0.72}$ & $-$\\
$3$ & Sink+Prog & $\mathbf{0.0}$ & $0.0$ & $0.0001$  & $0.06$ & $\mathbf{0.24}$ & $0.0130$ &1734.96 & 0.9935& $0.02$ & $0.0$ & $0.0004$\\
$3$ & Sink & $0.0$ & $\mathbf{0.18}$ & $0.0001$ & $0.04$ & $0.06$ & $0.0120$ &4192.92 & 0.9960& $0.00$ & $0.08$ & $0.0004$\\


% \hlie
% online & $2.00$ & Sink & $0.84$ & $0.16$ & $51.30$ & $0.0002$\\
% online & $2.00$ & Sink+Prog & $0.78$ & $0.22$ & $28.52$ & $0.00$\\
% % online & $2.00$ & none & $0.24$ & $0.00$ & $12.06$ & $0.00$\\
% offline & $2.00$ & $-$ & $0.00$ & $0.00$ & $10.58$  & $0.00$\\
% \hline
% offline & $3.00$ & $-$ & $0.72$ & $0.00$ & $13.76$ & $0.00$\\
% online & $3.00$ & Sink & $0.18$ & $0.82$ & $93.32$ & $0.0001$\\
% % online & $3.00$ & none & $0.00$ & $0.00$ & $6.02$ & $0.00$\\
% online & $3.00$ & Sink+Prog & $0.00$ & $1.00$ & $100.00$ & $0.0001$\
% online & $3.00$ & $dfa$ & $0.04$ & $51.84$ & $-$ & $0.00$ & $0.0008$ & $\infty$ & $0.0002$\\
% online & $3.00$ & none & $0.00$ & $5.56$ & $-$ & $0.00$ & $0.00$ & $\infty$ & $0.0001$\\
% online & $3.00$ & $dfa+pimdp$ & $0.00$ & $40.36$ & $-$ & $0.00$ & $0.00$ & $\infty$ & $0.0002$\\
% offline & $-$ & $3.00$ & $-$ & $0.00$ & $20.60$ &  - &  - & $\infty$ & $\infty$ & $0.00$\\
\end{tabular}


==> results/benchmark-prim-table.tex <==
\begin{tabular}{ccccccccc}
\hline
$Type$ & $1st Metric$ & $X_0$ & $2nd Metric$ & $Probability$ & $AvgSteps$ & $AvgImprove$ & $Avg1st$ & $Avg2nd$\\
\hline
$online$ & $worst - exp - lb$ & $1.00$ & $none$ & $1.00$ & $7.15$ & $0.00$ & $0.53$ & $\infty$\\
$online$ & $worst - exp - lb$ & $1.00$ & $worst - exp - ub$ & $1.00$ & $7.11$ & $0.00$ & $0.53$ & $\infty$\\
$online$ & $worst - exp - sum$ & $1.00$ & $none$ & $1.00$ & $7.15$ & $0.00$ & $1.35$ & $\infty$\\
$offline$ & $nil$ & $1.00$ & $nil$ & $1.00$ & $7.13$ & $\infty$ & $\infty$ & $\infty$\\
\hline
$online$ & $worst - exp - lb$ & $2.00$ & $worst - exp - ub$ & $1.00$ & $5.00$ & $0.00$ & $1.00$ & $\infty$\\
$online$ & $worst - exp - sum$ & $2.00$ & $none$ & $1.00$ & $5.00$ & $0.00$ & $1.25$ & $\infty$\\
$offline$ & $nil$ & $2.00$ & $nil$ & $1.00$ & $5.00$ & $\infty$ & $\infty$ & $\infty$\\
$online$ & $worst - exp - lb$ & $2.00$ & $none$ & $0.00$ & $4.00$ & $0.00$ & $0.00$ & $\infty$\\
\hline
$online$ & $worst - exp - lb$ & $3.00$ & $worst - exp - ub$ & $0.53$ & $13.16$ & $0.00$ & $0.07$ & $\infty$\\
$online$ & $worst - exp - sum$ & $3.00$ & $none$ & $0.45$ & $14.17$ & $0.00$ & $1.01$ & $\infty$\\
$online$ & $worst - exp - lb$ & $3.00$ & $none$ & $0.00$ & $2.00$ & $0.00$ & $0.00$ & $\infty$\\
$offline$ & $nil$ & $3.00$ & $nil$ & $0.00$ & $10.00$ & $\infty$ & $\infty$ & $\infty$\\
\hline
$online$ & $worst - exp - lb$ & $4.00$ & $none$ & $0.00$ & $2.00$ & $0.00$ & $0.00$ & $\infty$\\
$online$ & $worst - exp - lb$ & $4.00$ & $worst - exp - ub$ & $0.00$ & $4.00$ & $0.00$ & $0.00$ & $0.67$\\
$online$ & $worst - exp - sum$ & $4.00$ & $none$ & $0.00$ & $4.00$ & $0.00$ & $0.67$ & $\infty$\\
$offline$ & $nil$ & $4.00$ & $nil$ & $0.00$ & $4.00$ & $\infty$ & $\infty$ & $\infty$\\
\hline
$online$ & $worst - exp - lb$ & $5.00$ & $none$ & $0.00$ & $3.00$ & $0.00$ & $0.00$ & $\infty$\\
$online$ & $worst - exp - lb$ & $5.00$ & $worst - exp - ub$ & $0.00$ & $3.00$ & $0.00$ & $0.00$ & $0.00$\\
$online$ & $worst - exp - sum$ & $5.00$ & $none$ & $0.00$ & $3.00$ & $0.00$ & $0.00$ & $\infty$\\
$offline$ & $nil$ & $5.00$ & $nil$ & $0.00$ & $6.00$ & $\infty$ & $\infty$ & $\infty$\\
\end{tabular}


==> results/benchmark-table-global.tex <==
\begin{tabular}{cccccccccc}
$Type$ & $Met1$ & $Index$ & $SecRewardType$ & $Probability$ & $AverageRuns$ & $PolImprove$ & $1st Met$ & $2nd Met$ & $Time$\\
$online$ & $sum$ & $1.0000$ & $worst - dfa$ & $1.0000$ & $14.9000$ & $0$ & $1.0720$ & $\infty$ & $0.0002$\\
$online$ & $sum$ & $1.0000$ & $none$ & $0.8000$ & $48.0000$ & $0$ & $1.0609$ & $\infty$ & $0.0002$\\
$online$ & $lb$ & $1.0000$ & $none$ & $0.7000$ & $15.8000$ & $0$ & $0.0538$ & $\infty$ & $0.0002$\\
$online$ & $lb$ & $1.0000$ & $worst - dfa$ & $0.6000$ & $88.9000$ & $0$ & $0.0434$ & $\infty$ & $0.0002$\\
$online$ & $sum$ & $1.0000$ & $pimdp - metric1$ & $0.0000$ & $182.3000$ & $0$ & $1.0000$ & $2.9799$ & $0.0287$\\
$online$ & $sum$ & $1.0000$ & $worst - dfa - pimdp - metric1$ & $0.0000$ & $200.0000$ & $0$ & $1.0000$ & $\infty$ & $0.0114$\\
$online$ & $lb$ & $1.0000$ & $worst - dfa - pimdp - metric1$ & $0.0000$ & $200.0000$ & $0$ & $0.0000$ & $\infty$ & $0.0113$\\
$offline$ & $nil$ & $1.0000$ & $nil$ & $0.0000$ & $20.5000$ & $\infty$ & $\infty$ & $\infty$ & $0.0000$\\
$online$ & $sum$ & $2.0000$ & $worst - dfa$ & $1.0000$ & $14.0000$ & $0$ & $1.0790$ & $-1.1581$ & $0.0002$\\
$online$ & $lb$ & $2.0000$ & $worst - dfa$ & $1.0000$ & $13.5000$ & $0$ & $0.0824$ & $-1.1648$ & $0.0002$\\
$online$ & $sum$ & $2.0000$ & $none$ & $0.9000$ & $40.0000$ & $0$ & $1.0103$ & $\infty$ & $0.0007$\\
$online$ & $sum$ & $2.0000$ & $worst - dfa - pimdp - metric1$ & $0.7000$ & $142.4000$ & $0$ & $1.0073$ & $\infty$ & $0.0129$\\
$online$ & $lb$ & $2.0000$ & $worst - dfa - pimdp - metric1$ & $0.4000$ & $158.6000$ & $0$ & $0.0036$ & $\infty$ & $0.0140$\\
$online$ & $sum$ & $2.0000$ & $pimdp - metric1$ & $0.0000$ & $55.9000$ & $0$ & $0.9641$ & $2.4799$ & $0.0155$\\
$online$ & $lb$ & $2.0000$ & $none$ & $0.0000$ & $10.7000$ & $0$ & $0.0000$ & $\infty$ & $0.0002$\\
$offline$ & $nil$ & $2.0000$ & $nil$ & $0.0000$ & $11.2000$ & $\infty$ & $\infty$ & $\infty$ & $0.0000$\\
\end{tabular}


==> results/benchmark-table-local.tex <==
\begin{tabular}{cccccccccc}
$Type$ & $Met1$ & $Index$ & $SecRewardType$ & $Probability$ & $AverageRuns$ & $PolImprove$ & $1st Met$ & $2nd Met$ & $Time$\\
$online$ & $sum$ & $1.0000$ & $worst - dfa$ & $1.0000$ & $14.6000$ & $0.0000$ & $0.5368$ & $\infty$ & $0.0032$\\
$online$ & $lb$ & $1.0000$ & $worst - dfa$ & $1.0000$ & $14.8000$ & $0.0000$ & $0.0725$ & $\infty$ & $0.0035$\\
$online$ & $sum$ & $1.0000$ & $none$ & $0.2000$ & $161.7000$ & $0.0000$ & $0.5074$ & $\infty$ & $0.0022$\\
$online$ & $lb$ & $1.0000$ & $none$ & $0.1000$ & $19.4000$ & $0.0000$ & $0.0077$ & $\infty$ & $0.0028$\\
$online$ & $sum$ & $1.0000$ & $pimdp - metric1$ & $0.0000$ & $200.0000$ & $0.0000$ & $0.5000$ & $2.9890$ & $0.0417$\\
$online$ & $sum$ & $1.0000$ & $worst - dfa - pimdp - metric1$ & $0.0000$ & $200.0000$ & $0.0000$ & $0.5000$ & $\infty$ & $0.0199$\\
$online$ & $lb$ & $1.0000$ & $worst - dfa - pimdp - metric1$ & $0.0000$ & $200.0000$ & $0.0000$ & $0.0000$ & $\infty$ & $0.0197$\\
$offline$ & $nil$ & $1.0000$ & $nil$ & $0.0000$ & $20.2000$ & $\infty$ & $\infty$ & $\infty$ & $0.0000$\\
$online$ & $sum$ & $2.0000$ & $worst - dfa$ & $1.0000$ & $37.2000$ & $0.0000$ & $0.5215$ & $\infty$ & $0.0022$\\
$online$ & $lb$ & $2.0000$ & $worst - dfa$ & $0.4000$ & $24.9000$ & $0.0000$ & $0.0173$ & $\infty$ & $0.0021$\\
$online$ & $sum$ & $2.0000$ & $none$ & $0.0000$ & $30.4000$ & $0.0000$ & $0.4200$ & $\infty$ & $0.0019$\\
$online$ & $sum$ & $2.0000$ & $pimdp - metric1$ & $0.0000$ & $64.2000$ & $0.0000$ & $0.4706$ & $2.3788$ & $0.0237$\\
$online$ & $sum$ & $2.0000$ & $worst - dfa - pimdp - metric1$ & $0.0000$ & $200.0000$ & $0.0000$ & $0.5000$ & $2.3175$ & $0.0194$\\
$online$ & $lb$ & $2.0000$ & $none$ & $0.0000$ & $10.4000$ & $0.0000$ & $0.0000$ & $\infty$ & $0.0033$\\
$online$ & $lb$ & $2.0000$ & $worst - dfa - pimdp - metric1$ & $0.0000$ & $200.0000$ & $0.0000$ & $0.0000$ & $2.4130$ & $0.0073$\\
$offline$ & $nil$ & $2.0000$ & $nil$ & $0.0000$ & $11.5000$ & $\infty$ & $\infty$ & $\infty$ & $0.0000$\\
\end{tabular}


==> results/benchmark-table.tex <==
\begin{tabular}{ccccccccc}
\hline
$Type$ & $1st Metric$ & $X_0$ & $2nd Metric$ & $Probability$ & $AvgSteps$ & $AvgImprove$ & $Avg1st$ & $Avg2nd$\\
\hline
$online$ & $worst - exp - sum$ & $1.00$ & $none$ & $1.00$ & $7.09$ & $0.00$ & $1.34$ & $\infty$\\
$online$ & $worst - exp - sum$ & $1.00$ & $worst - dfa$ & $1.00$ & $10.19$ & $0.00$ & $1.24$ & $\infty$\\
$online$ & $worst - exp - sum$ & $1.00$ & $expected - dfa$ & $1.00$ & $7.06$ & $0.00$ & $1.34$ & $\infty$\\
$offline$ & $nil$ & $1.00$ & $nil$ & $1.00$ & $7.08$ & $\infty$ & $\infty$ & $\infty$\\
$online$ & $worst - exp - sum$ & $1.00$ & $exp - probs$ & $0.97$ & $8.87$ & $0.00$ & $1.32$ & $\infty$\\
$online$ & $worst - exp - sum$ & $2.00$ & $none$ & $1.00$ & $5.00$ & $0.00$ & $1.25$ & $\infty$\\
$online$ & $worst - exp - sum$ & $2.00$ & $worst - dfa$ & $1.00$ & $5.00$ & $0.00$ & $1.25$ & $\infty$\\
$online$ & $worst - exp - sum$ & $2.00$ & $exp - probs$ & $1.00$ & $5.00$ & $0.00$ & $1.25$ & $\infty$\\
$offline$ & $nil$ & $2.00$ & $nil$ & $1.00$ & $5.00$ & $\infty$ & $\infty$ & $\infty$\\
$online$ & $worst - exp - sum$ & $2.00$ & $expected - dfa$ & $0.00$ & $2.00$ & $0.00$ & $0.00$ & $0.00$\\
$online$ & $worst - exp - sum$ & $3.00$ & $worst - dfa$ & $1.00$ & $6.03$ & $0.00$ & $1.20$ & $\infty$\\
$online$ & $worst - exp - sum$ & $3.00$ & $none$ & $0.00$ & $4.00$ & $0.00$ & $0.67$ & $\infty$\\
$online$ & $worst - exp - sum$ & $3.00$ & $expected - dfa$ & $0.00$ & $4.00$ & $0.00$ & $0.67$ & $\infty$\\
$online$ & $worst - exp - sum$ & $3.00$ & $exp - probs$ & $0.00$ & $4.00$ & $0.00$ & $0.67$ & $1.33$\\
$offline$ & $nil$ & $3.00$ & $nil$ & $0.00$ & $4.00$ & $\infty$ & $\infty$ & $\infty$\\
$online$ & $worst - exp - sum$ & $4.00$ & $expected - dfa$ & $1.00$ & $13.07$ & $0.00$ & $1.09$ & $NaN$\\
$online$ & $worst - exp - sum$ & $4.00$ & $worst - dfa$ & $0.94$ & $10.98$ & $0.00$ & $1.09$ & $\infty$\\
$online$ & $worst - exp - sum$ & $4.00$ & $none$ & $0.44$ & $13.29$ & $0.00$ & $1.01$ & $\infty$\\
$online$ & $worst - exp - sum$ & $4.00$ & $exp - probs$ & $0.42$ & $14.51$ & $0.00$ & $1.00$ & $\infty$\\
$offline$ & $nil$ & $4.00$ & $nil$ & $0.00$ & $10.00$ & $\infty$ & $\infty$ & $\infty$\\
$online$ & $worst - exp - sum$ & $5.00$ & $exp - probs$ & $0.82$ & $5.46$ & $0.00$ & $0.82$ & $\infty$\\
$online$ & $worst - exp - sum$ & $5.00$ & $none$ & $0.00$ & $3.00$ & $0.00$ & $0.00$ & $\infty$\\
$online$ & $worst - exp - sum$ & $5.00$ & $worst - dfa$ & $0.00$ & $3.00$ & $0.00$ & $0.00$ & $\infty$\\
$online$ & $worst - exp - sum$ & $5.00$ & $expected - dfa$ & $0.00$ & $3.00$ & $0.00$ & $0.00$ & $0.00$\\
$offline$ & $nil$ & $5.00$ & $nil$ & $0.00$ & $5.97$ & $\infty$ & $\infty$ & $\infty$\\
\end{tabular}

